Van Kampen Colimits and Path Uniqueness

Fibred semantics is the foundation of the model-instance pattern of software engineering. Software models can often be formalized as objects of presheaf topoi, i.e, categories of objects that can be represented as algebras as well as coalgebras, e.g., the category of directed graphs. Multimodeling requires to construct colimits of models, decomposition is given by pullback. Compositionality requires an exact interplay of these operations, i.e., diagrams must enjoy the Van Kampen property. However, checking the validity of the Van Kampen property algorithmically based on its definition is often impossible. In this paper we state a necessary and sufficient yet efficiently checkable condition for the Van Kampen property to hold in presheaf topoi. It is based on a uniqueness property of path-like structures within the defining congruence classes that make up the colimiting cocone of the models. We thus add to the statement "Being Van Kampen is a Universal Property" by Heindel and Soboci\'{n}ski the fact that the Van Kampen property reveals a presheaf-based structural uniqueness feature.

==> 6-sect6.tex <==
\subsection{Checking for Cyclic Mapping Paths only}
All conditions in Corollary \ref{cor:main} are equivalent to 
\begin{equation}\label{equ:proper-cycle-condition}
  \forall z:\mbox{ There is no non-empty proper mapping path connecting $z$ with itself},
\end{equation}
because on the one hand any cyclic proper non-empty mapping path from $z$ to itself is accompanied by the empty path from $z$ to itself. On the other hand, if $z\not= z'$, the existence of two disjoint proper mapping paths in $\FD$ connecting $z$ and $z'$ provides a non-empty proper mapping path connecting $z$ with itself since the first path can be composed with the reversed second path. This composition becomes proper again since the paths are disjoint.
\par 
If $\I$ has no directed cycles, we will show now that it is even enough to check only the branching components for cyclic mapping paths. Note, that this criterion generalizes smoothly our original condition in Theorem \ref{theo:VK-pushout} for VK pushouts. In the same way as Theorem \ref{theo:main_minimal}, this criterion is also useful in practice, because, again, one can reduce analysis to presumably small branching components.
\par 
We consider a non-empty mapping path $P=[(y_0, \delta_0, y_1), (y_1, \delta_1, y_2), \ldots, (y_{n-1},\delta_{n-1}, y_n)]$ with $y_0=y_n$. If $\iota_0\notin Br(\I)$ we can not have $\delta_{n-1}\in\I_1^{op}$ and $\delta_0\in\I_1$ at the same time. Since there is no loop in $\I$ we have $n\geq 2$. Moreover, since there are no directed cycles in $\I$ at least one of the $\delta_i$'s must be in $\I_1$ and at least one in $\I_1^{op}$. In such a way, there must be at least one branching position $j$ with $0< j < n$, i.e.\ $\iota_j$ is a branching index. Thus the cycle can be transformed into a non-empty cyclic proper mapping path connecting $y_j$ in $\FD_{\iota_j}(X)$ with itself where $\iota_j\in Br(\I)$. This shows that we need to check condition \myref{equ:proper-cycle-condition} indeed only for branching indices. Note, that we have, in such a way, another argument, now based on Corollary  \ref{cor:main}, that we have VK for free if there is no branching in our finite $\I$ without directed cycles!
\par
Due to inner-cycle reduction (Lemma \ref{fact7}) it would be even enough to check the existence of cyclic non-empty inner-cycle free and proper mapping paths for elements in branching components. This yields
\begin{thm}[Non-Empty Cyclic Paths]\label{theo:main_cycles}
Let $\G = \pre{\B}$ be a presheaf topos and $\FD:\I\to\G$ be a diagram with $\I$ a finite directed multigraph without directed cycles. Let
\[\FD\stackrel{\kappa}{\Rightarrow} \Delta S\]
be a colimiting cocone. The following are equivalent: 
\[\begin{array}{clll}
(1) & \mbox{The cocone is VK} & &\\
(2) & \forall X\in \B, i\in Br(\I), z\in\FD_i(X): &
\mbox{There is no non-empty proper mapping path from $z$ to itself} &\\
(2) & \forall X\in \B, i\in Br(\I), z\in\FD_i(X):& 
\mbox{There is no non-empty inner-cycle free and proper mapping} &\\
&& \mbox{path from $z$ to itself }\hfill &\\
\end{array}
\]
\end{thm}
In Fig.\ref{fig:decision-diagram} it is now possible to omit the check for image-disjointness and carry out the algorithm according to Theorem \ref{theo:main_cycles} after having checked for directed cyles and branching in $\I$. In Fig.\ref{fig:example1}, it is easy to see that the cyclic path 
\[(Sort,d_{-13}^{op},S/I),(S/I, d_{13}, Intf.),(Intf., d_{23}^{op},T/I), (T/I,d_{-23},Type), (Type, d_{12}^{op}, S/T), (S/T, d_{-12}, Sort)\]
is the witness for VK violation. Not surprisingly, it is the concatenation of the two indicating paths already given in Sect.\ref{sec:appl}.
\par 
The methodology of the present section, however, is not directly combinable with colimit computation, since the algorithm of Sect.\ref{sec:dec-diagram} collects pairs in minimal components only, while cyclic path construction takes place in arbitrary components. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ms.tex"
%%% End:

